Short time-scale optical variability properties of the largest AGN sample observed with Kepler/K2

We present the first short time-scale ($\sim$hours to days) optical variability study of a large sample of Active Galactic Nuclei (AGN) observed with the Kepler/K2 mission. The sample contains 252 AGN observed over four campaigns with $\sim 30$ minute cadence selected from the Million Quasar Catalogue with R magnitude $< 19$. We performed time series analysis to determine their variability properties by means of the power spectral densities (PSDs) and applied Monte Carlo techniques to find the best model parameters that fit the observed power spectra. A power-law model is sufficient to describe all the PSDs of our sample. A variety of power-law slopes were found indicating that there is not a universal slope for all AGN. We find that the rest-frame amplitude variability in the frequency range of $6\times10^{-6}-10^{-4}$ Hz varies from $1-10$ % with an average of 1.7 %. We explore correlations between the variability amplitude and key parameters of the AGN, finding a significant correlation of rest-frame short-term variability amplitude with redshift. We attribute this effect to the known "bluer when brighter" variability of quasars combined with the fixed bandpass of Kepler data. This study also enables us to distinguish between Seyferts and Blazars and confirm AGN candidates. For our study we have compared results obtained from light curves extracted using different aperture sizes and with and without de-trending. We find that limited de-trending of the optimal photometric precision light curve is the best approach, although some systematic effects still remain present.

==> latextable_12novmoire.tex <==
201146408&174.5331&-5.3805&q&19.4&18.4&2.00&$2.18^{+0.82}_{-1.08}$&$1.66^{+0.70}_{-0.64}$&$1.39^{+1.41}_{-1.40}$&0.46&1.54&36.9&1.12&1.06&$1.32\pm0.12$&326.25\\
201150761&174.7086&-5.2778&q&18.5&18.2&1.20&$2.84^{+0.60}_{-0.67}$&$1.79^{+1.15}_{-1.15}$&$2.71^{+0.68}_{-1.40}$&4.68&0.71&90.7&0.76&0.66&$1.29\pm0.52$&190.46\\
201153744&172.1308&-5.2070&q&18.5&18.2&1.10&$1.92^{+0.97}_{-0.35}$&$1.92^{+0.70}_{-0.31}$&$1.53^{+0.70}_{-0.69}$&1.16&0.60&44.2&0.82&0.84&$1.02\pm0.09$&153.57\\
201157230&173.9066&-5.1233&q&18.3&17.7&1.00&$2.58^{+0.71}_{-0.71}$&$2.45^{+0.00}_{-0.00}$&$2.32^{+0.69}_{-0.69}$&3.68&0.32&74.2&1.13&1.07&$1.69\pm0.38$&145.13\\
201167738&173.0793&-4.8731&q&19.2&18.5&1.40&$2.84^{+0.54}_{-0.44}$&$2.58^{+0.00}_{-0.00}$&$2.71^{+0.44}_{-0.43}$&5.79&1.38&27.8&2.58&2.54&$5.36\pm0.83$&157.59\\
201169297&172.6518&-4.8334&q&19.4&18.0&1.50&$1.79^{+1.41}_{-0.71}$&$2.18^{+1.19}_{-1.19}$&$1.66^{+1.44}_{-0.46}$&1.08&1.01&33.8&0.74&0.76&$1.03\pm0.13$&161.06\\
201169810&169.7321&-4.8214&R&18.3&17.8&0.00&$3.24^{+0.50}_{-0.50}$&$2.45^{+0.58}_{-1.03}$&$1.92^{+0.00}_{-0.00}$&2.73&0.20&8.9&0.92&0.91&$0.00\pm0.00$&0.00\\
201184312&173.9927&-4.4744&AR&18.7&17.0&0.27&$1.66^{+0.34}_{-0.44}$&$1.66^{+0.35}_{-0.38}$&$1.53^{+0.41}_{-0.41}$&1.72&-15.53&76.6&25.71&24.83&$26.45\pm2.25$&0.00\\
201184625&176.5165&-4.4670&AX&16.6&15.4&0.13&$3.11^{+0.77}_{-0.77}$&$2.97^{+0.79}_{-0.79}$&$2.58^{+0.27}_{-0.28}$&4.92&0.04&16.2&0.70&0.65&$0.71\pm0.14$&5.22\\
201185828&173.2443&-4.4373&q&19.1&18.4&1.60&$2.58^{+0.56}_{-0.70}$&$2.18^{+0.48}_{-0.37}$&$2.45^{+0.57}_{-0.57}$&4.39&0.35&79.6&1.80&1.78&$3.55\pm0.56$&5.94\\
201187307&172.3197&-4.4020&AR&14.1&13.3&0.06&$2.45^{+0.63}_{-0.65}$&$2.58^{+0.60}_{-0.83}$&$2.32^{+0.63}_{-0.46}$&3.94&0.01&88.7&0.69&0.66&$0.69\pm0.23$&246.74\\
201189418&173.3896&-4.3509&q&19.1&18.5&2.50&$2.45^{+0.60}_{-0.69}$&$2.18^{+0.33}_{-0.43}$&$2.45^{+0.57}_{-0.70}$&4.25&0.62&94.6&2.44&2.53&$6.25\pm0.82$&0.00\\
201193441&175.3808&-4.2557&q&18.2&17.9&1.10&$2.84^{+0.65}_{-0.98}$&$2.97^{+0.36}_{-1.17}$&$2.71^{+0.40}_{-0.83}$&5.35&0.20&21.5&0.58&0.54&$1.02\pm0.26$&8.99\\
201197637&174.7716&-4.1574&q&20.0&18.5&1.60&$3.37^{+0.00}_{-0.00}$&$2.18^{+1.25}_{-1.25}$&$1.66^{+0.00}_{-0.00}$&0.97&1.01&8.6&0.91&0.90&$1.24\pm0.00$&197.89\\
201197767&172.9189&-4.1548&qX&17.8&17.7&0.30&$2.45^{+0.00}_{-0.00}$&$2.05^{+0.89}_{-1.03}$&$2.84^{+0.00}_{-0.00}$&5.63&0.28&8.4&1.38&1.26&$1.60\pm0.00$&115.39\\
201207010&170.8428&-3.9385&QX&17.5&17.8&0.37&$2.32^{+0.51}_{-0.45}$&$2.45^{+0.00}_{-0.00}$&$2.05^{+0.57}_{-0.36}$&3.07&0.15&58.9&1.50&1.35&$1.59\pm0.29$&13.15\\
201209205&175.6203&-3.8866&q&18.7&17.9&0.50&$2.84^{+0.82}_{-0.82}$&$2.58^{+0.69}_{-1.03}$&$2.32^{+0.62}_{-0.56}$&4.12&0.16&78.8&0.67&0.72&$0.94\pm0.24$&26.33\\
201215807&173.8962&-3.7336&QR&16.8&14.8&1.16&$2.71^{+0.36}_{-0.93}$&$2.32^{+0.41}_{-0.50}$&$1.26^{+0.18}_{-0.24}$&0.41&0.00&17.0&0.09&0.10&$0.11\pm0.00$&20.77\\
201219689&176.3963&-3.6670&BR&18.8&16.4&0.17&$2.97^{+0.33}_{-0.83}$&$2.58^{+0.57}_{-0.65}$&$1.66^{+0.46}_{-0.42}$&2.06&0.05&78.1&0.68&0.71&$0.74\pm0.09$&749.86\\
201219871&176.2966&-3.6639&AX&19.2&18.4&0.37&$3.11^{+0.37}_{-0.76}$&$2.71^{+0.65}_{-0.64}$&$2.84^{+0.51}_{-0.76}$&5.24&0.58&60.4&1.75&1.72&$2.31\pm0.99$&1.74\\
201222389&173.6438&-3.6240&QR&18.5&18.2&2.07&$2.58^{+0.46}_{-1.20}$&$1.92^{+1.15}_{-0.89}$&$2.84^{+0.00}_{-0.00}$&5.28&0.23&6.0&0.34&0.31&$0.86\pm0.00$&7.03\\
201225977&176.1200&-3.5709&AR&15.0&12.1&0.05&$2.71^{+0.51}_{-0.87}$&$2.45^{+0.48}_{-0.84}$&$1.79^{+0.53}_{-0.59}$&2.43&0.00&59.2&0.16&0.17&$0.17\pm0.04$&763.94\\
201226680&173.3356&-3.5605&AR&17.6&16.1&0.12&$2.84^{+0.07}_{-0.31}$&$2.84^{+0.63}_{-1.03}$&$1.39^{+0.58}_{-0.57}$&0.36&0.03&44.8&0.24&0.25&$0.26\pm0.03$&2.95\\
201232832&170.0653&-3.4689&q&18.9&18.3&1.90&$2.32^{+0.25}_{-0.24}$&$1.92^{+0.00}_{-0.00}$&$2.18^{+0.00}_{-0.00}$&3.49&0.45&4.6&2.21&1.96&$3.68\pm0.00$&2.16\\
201239441&178.6183&-3.3697&q&19.9&18.2&0.20&$2.71^{+0.56}_{-1.07}$&$1.92^{+0.55}_{-0.55}$&$2.32^{+0.63}_{-1.11}$&3.09&0.67&82.4&0.90&0.74&$0.83\pm0.40$&445.24\\
201240157&172.2191&-3.3585&KR&17.8&16.6&0.20&$2.84^{+0.50}_{-0.79}$&$2.05^{+0.81}_{-0.86}$&$2.45^{+0.61}_{-0.67}$&4.58&0.08&66.3&0.77&0.73&$0.83\pm0.32$&1.08\\
201246403&170.8579&-3.2635&QR&17.9&17.6&1.77&$2.84^{+0.53}_{-0.86}$&$2.18^{+0.07}_{-0.11}$&$2.84^{+0.49}_{-0.96}$&5.39&0.15&63.6&1.05&1.05&$2.69\pm0.64$&5.25\\
201246601&179.4717&-3.2603&AR&15.8&15.5&0.21&$2.05^{+0.96}_{-0.96}$&$2.84^{+0.49}_{-0.90}$&$2.32^{+0.77}_{-0.77}$&4.75&0.05&94.9&0.56&0.58&$0.66\pm0.27$&887.31\\
201250126&169.9206&-3.2053&q&18.5&18.1&1.10&$2.32^{+0.41}_{-0.25}$&$1.79^{+0.50}_{-0.36}$&$2.05^{+0.00}_{-0.00}$&3.51&0.47&2.7&1.87&1.56&$2.30\pm0.00$&31.24\\
201255940&178.2156&-3.1174&q&19.2&18.4&1.30&$2.18^{+0.59}_{-0.59}$&$2.05^{+0.00}_{-0.00}$&$1.79^{+0.83}_{-0.69}$&1.74&1.11&80.8&1.11&1.12&$1.56\pm0.20$&153.57\\
201261416&179.7416&-3.0354&R&18.6&18.0&0.00&$2.71^{+0.43}_{-0.40}$&$2.84^{+1.25}_{-1.25}$&$1.66^{+0.81}_{-0.81}$&0.88&0.49&38.8&0.60&0.52&$0.00\pm0.00$&0.00\\
201263046&178.4697&-3.0103&AR&18.7&17.4&0.20&$2.71^{+0.50}_{-0.45}$&$1.26^{+1.25}_{-1.25}$&$2.18^{+0.82}_{-0.78}$&3.00&0.37&25.8&0.49&0.38&$0.42\pm0.16$&128.78\\
201272471&169.9118&-2.8675&Q&17.9&17.5&0.66&$2.84^{+0.00}_{-0.00}$&$2.18^{+0.00}_{-0.00}$&$2.84^{+0.00}_{-0.00}$&6.07&0.29&0.9&1.55&1.36&$2.17\pm0.00$&2.64\\
201336263&179.7133&-1.9118&QR&18.3&18.0&1.90&$3.11^{+0.99}_{-0.99}$&$2.32^{+0.74}_{-0.99}$&$2.58^{+0.61}_{-1.33}$&4.57&0.49&72.4&0.74&0.72&$1.66\pm0.44$&78.58\\
201340127&172.9193&-1.8551&AX&18.7&18.1&0.43&$2.58^{+0.59}_{-0.65}$&$2.45^{+0.68}_{-1.25}$&$2.71^{+0.52}_{-0.78}$&5.36&0.23&81.8&1.02&1.09&$1.49\pm0.58$&741.98\\
201343412&179.6894&-1.8059&AR&17.3&15.5&0.09&$3.37^{+0.64}_{-0.64}$&$2.58^{+0.53}_{-0.71}$&$1.39^{+0.00}_{-0.00}$&0.86&0.08&6.7&0.37&0.41&$0.42\pm0.00$&14.88\\
201345754&178.8811&-1.7700&QX&20.7&18.5&3.19&$2.97^{+0.51}_{-0.64}$&$3.24^{+0.00}_{-0.00}$&$2.58^{+0.46}_{-0.67}$&5.26&1.05&41.8&2.21&1.98&$6.13\pm0.65$&0.00\\
201346523&169.7585&-1.7579&QR&18.8&18.3&1.30&$1.92^{+0.63}_{-0.63}$&$2.05^{+0.65}_{-0.50}$&$1.79^{+0.74}_{-0.63}$&1.54&19.23&77.8&4.83&4.78&$6.65\pm0.78$&1.55\\
201350814&171.6695&-1.6938&AR&13.5&11.8&0.05&$3.24^{+1.21}_{-1.21}$&$2.32^{+0.68}_{-0.68}$&$1.66^{+0.56}_{-0.38}$&1.48&0.00&38.2&0.08&0.08&$0.09\pm0.01$&180.42\\
201352437&178.3481&-1.6691&R&19.8&18.5&0.00&$2.18^{+0.53}_{-0.48}$&$2.32^{+0.27}_{-0.01}$&$1.92^{+0.36}_{-0.15}$&2.47&0.26&19.1&1.74&1.48&$0.00\pm0.00$&0.00\\
201354965&172.4329&-1.6312&QX&18.5&18.1&1.29&$3.11^{+1.08}_{-1.08}$&$1.66^{+0.38}_{-0.37}$&$2.71^{+0.65}_{-1.19}$&4.97&0.17&64.6&0.46&0.44&$0.90\pm0.31$&8.79\\
201356907&170.9271&-1.6017&AR&16.3&14.5&0.06&$2.58^{+0.96}_{-0.96}$&$2.32^{+0.50}_{-0.70}$&$2.18^{+0.76}_{-0.75}$&3.45&0.01&80.9&0.13&0.14&$0.14\pm0.06$&229.96\\
201362181&172.4700&-1.5245&QX&18.1&18.2&0.48&$2.58^{+0.67}_{-0.84}$&$2.32^{+0.75}_{-0.92}$&$2.71^{+0.61}_{-0.90}$&5.54&0.11&83.5&0.78&0.76&$1.06\pm0.46$&1.78\\
201365301&173.1494&-1.4802&Q2&18.4&18.1&0.44&$2.58^{+0.55}_{-0.66}$&$2.05^{+0.67}_{-0.84}$&$2.45^{+0.49}_{-0.73}$&4.92&0.48&55.0&1.40&1.39&$1.80\pm0.55$&31.26\\
201367243&179.9207&-1.4523&QR&18.4&18.2&1.21&$2.45^{+0.69}_{-0.89}$&$2.84^{+0.55}_{-0.72}$&$2.45^{+0.48}_{-1.18}$&4.00&0.72&30.4&0.53&0.48&$0.86\pm0.23$&19.66\\
201373523&172.4418&-1.3613&QR&17.5&17.7&0.73&$3.24^{+0.89}_{-0.89}$&$2.05^{+0.08}_{-0.26}$&$2.18^{+1.04}_{-0.55}$&4.14&0.05&53.3&0.65&0.64&$0.88\pm0.24$&212.50\\
201380932&166.6533&-1.2485&QR&17.7&16.6&1.00&$2.97^{+0.53}_{-1.09}$&$1.92^{+0.72}_{-0.80}$&$2.71^{+0.63}_{-1.18}$&5.03&0.10&92.6&0.57&0.57&$1.04\pm0.40$&136.28\\
201405115&166.6324&-0.8812&QR&16.1&16.0&0.42&$3.11^{+0.39}_{-0.55}$&$2.97^{+0.93}_{-0.94}$&$2.05^{+0.89}_{-0.86}$&2.83&0.07&87.0&0.31&0.30&$0.36\pm0.12$&241.70\\
201435637&168.1297&-0.4262&QR&18.4&18.5&0.54&$3.24^{+0.40}_{-0.40}$&$2.97^{+0.39}_{-0.62}$&$3.24^{+0.54}_{-0.54}$&6.35&0.45&21.7&1.19&1.17&$1.90\pm0.75$&118.83\\
201437504&177.6828&-0.3984&QR&17.7&17.2&1.98&$3.37^{+0.55}_{-0.55}$&$1.66^{+0.00}_{-0.00}$&$1.79^{+0.92}_{-0.92}$&2.54&0.04&79.4&0.42&0.43&$0.66\pm0.08$&32.39\\
201438859&168.2943&-0.3784&QR&18.1&17.9&1.12&$2.84^{+0.51}_{-1.23}$&$2.32^{+0.96}_{-1.14}$&$2.58^{+0.53}_{-1.15}$&4.10&0.21&55.4&0.67&0.62&$1.12\pm0.35$&1381.04\\
201441589&168.5081&-0.3385&q&18.8&18.4&1.20&$2.84^{+0.53}_{-1.00}$&$2.18^{+0.57}_{-0.76}$&$3.11^{+0.00}_{-0.00}$&5.70&0.82&8.6&2.04&1.82&$4.17\pm0.00$&224.23\\
201455836&168.5412&-0.1358&AR&17.2&15.7&0.10&$2.84^{+0.42}_{-0.78}$&$2.58^{+0.48}_{-0.88}$&$2.45^{+0.36}_{-0.44}$&3.90&0.06&33.7&0.47&0.49&$0.52\pm0.14$&147.84\\
201456026$^{*}$&171.2781&-0.1334&QX&17.9&18.0&1.91&$1.66^{+0.46}_{-0.37}$&$1.66^{+0.47}_{-0.52}$&$1.53^{+0.42}_{-0.40}$&1.50&0.12&61.8&0.78&0.81&$1.07\pm0.04$&2.14\\
201456561&168.4268&-0.1252&QR&19.3&18.5&1.55&$3.37^{+0.86}_{-0.86}$&$2.18^{+0.62}_{-0.60}$&$3.11^{+0.18}_{-0.18}$&6.59&1.02&14.1&1.27&1.15&$3.07\pm0.23$&1064.38\\
201466253$^{*}$&171.4262&0.0170&QR&17.6&17.4&1.69&$1.39^{+0.33}_{-0.33}$&$1.39^{+0.49}_{-0.34}$&$1.00^{+0.42}_{-0.42}$&-0.37&0.08&41.0&0.47&0.51&$0.51\pm0.00$&189.92\\
201466962&168.7520&0.0272&QX&18.9&18.2&1.33&$2.45^{+0.62}_{-0.52}$&$2.45^{+0.47}_{-0.73}$&$2.58^{+0.46}_{-0.71}$&5.09&0.71&51.9&1.62&1.64&$3.20\pm0.64$&1023.69\\
201479228&167.2854&0.2087&QR&17.9&17.9&0.54&$1.92^{+0.96}_{-0.40}$&$2.18^{+0.50}_{-0.66}$&$1.92^{+0.95}_{-0.51}$&2.79&0.08&66.7&0.65&0.66&$0.80\pm0.18$&176.79\\
201480698&176.6988&0.2307&QX&18.4&18.0&0.94&$2.71^{+0.57}_{-0.84}$&$2.18^{+0.58}_{-0.91}$&$2.18^{+0.65}_{-0.79}$&3.15&0.17&68.1&0.35&0.42&$0.63\pm0.14$&47.07\\
201499023&168.0909&0.5079&QR&18.3&18.4&0.52&$2.97^{+0.99}_{-0.99}$&$2.71^{+0.52}_{-0.99}$&$2.84^{+0.25}_{-0.43}$&5.82&0.34&18.6&1.44&1.41&$2.08\pm0.43$&115.71\\
201503438$^{*}$&173.1901&0.5743&QR&18.0&17.3&1.22&$2.45^{+0.66}_{-0.68}$&$2.05^{+0.71}_{-0.74}$&$2.05^{+0.33}_{-0.33}$&3.26&0.14&73.3&2.07&1.97&$3.00\pm0.24$&32.11\\
201524316&175.0695&0.8976&QR&19.0&18.3&1.14&$2.58^{+0.53}_{-0.73}$&$2.32^{+0.61}_{-0.57}$&$2.58^{+0.59}_{-0.73}$&4.81&0.03&90.2&0.53&0.53&$0.96\pm0.23$&305.48\\
201546147$^{*}$&175.9752&1.2287&QR&18.1&17.5&1.28&$2.84^{+0.00}_{-0.00}$&$2.84^{+0.59}_{-1.48}$&$2.71^{+0.00}_{-0.00}$&5.20&0.03&3.7&0.20&0.17&$0.34\pm0.00$&108.96\\
201548884&174.3733&1.2705&QR&19.5&17.9&0.43&$2.97^{+0.53}_{-0.78}$&$2.32^{+0.54}_{-0.76}$&$3.11^{+0.27}_{-0.60}$&6.66&0.10&26.0&0.87&0.82&$1.19\pm0.38$&312.09\\
201550049&170.5392&1.2887&AX&17.5&16.4&0.06&$2.32^{+0.61}_{-0.47}$&$2.32^{+0.70}_{-0.60}$&$2.18^{+0.72}_{-0.30}$&3.53&-0.02&46.4&2.40&2.29&$2.37\pm0.68$&7.71\\
201555274&170.9025&1.3672&QR&18.7&18.4&0.94&$2.18^{+0.63}_{-0.63}$&$1.00^{+1.36}_{-1.36}$&$2.05^{+0.41}_{-0.53}$&2.71&0.34&36.8&0.71&0.71&$1.01\pm0.13$&0.62\\
201568886&168.8567&1.5686&AR&18.3&17.6&0.24&$2.58^{+0.79}_{-0.79}$&$2.05^{+0.64}_{-0.64}$&$2.45^{+0.69}_{-0.76}$&4.73&0.37&99.6&1.76&1.75&$2.04\pm0.87$&90.25\\
201569249&174.6333&1.5742&QX&18.4&17.9&0.38&$2.97^{+0.49}_{-1.03}$&$2.32^{+0.64}_{-0.86}$&$2.84^{+0.56}_{-1.01}$&5.31&0.10&82.3&1.14&1.13&$1.52\pm0.80$&5.30\\
201570346&168.0252&1.5901&AR&20.3&17.7&0.18&$2.97^{+0.60}_{-0.60}$&$2.58^{+0.00}_{-0.00}$&$1.39^{+0.00}_{-0.00}$&0.80&0.08&4.7&0.60&0.59&$0.61\pm0.00$&14.17\\
201572944&170.8364&1.6299&QX&15.3&15.5&1.47&$2.84^{+0.52}_{-0.93}$&$2.18^{+0.63}_{-0.75}$&$2.32^{+0.69}_{-0.87}$&3.54&0.01&94.9&0.16&0.16&$0.30\pm0.06$&0.68\\
201575185&174.2785&1.6633&QX&19.3&18.3&0.19&$2.97^{+0.43}_{-0.20}$&$3.24^{+0.21}_{-0.43}$&$2.18^{+0.65}_{-0.65}$&4.05&0.02&98.6&1.08&1.06&$1.18\pm0.38$&5328.23\\
201580937&170.2490&1.7491&BR&18.2&17.9&0.37&$2.84^{+0.64}_{-0.95}$&$1.92^{+0.84}_{-0.48}$&$1.79^{+1.03}_{-0.43}$&2.48&0.00&65.1&0.14&0.14&$0.16\pm0.03$&1.58\\
201581813&177.4353&1.7618&QX&18.5&18.3&1.47&$2.84^{+0.64}_{-1.00}$&$1.66^{+0.84}_{-0.84}$&$1.66^{+1.26}_{-0.49}$&1.55&0.12&49.7&0.42&0.46&$0.62\pm0.07$&15.16\\
201592923$^{*}$&176.6947&1.9345&QR&18.7&18.0&2.64&$2.32^{+0.67}_{-0.79}$&$1.53^{+0.71}_{-0.71}$&$1.92^{+0.77}_{-0.52}$&2.70&0.10&68.3&0.69&0.65&$1.18\pm0.10$&0.00\\
201595011&174.1327&1.9670&QX&18.7&18.3&1.47&$2.58^{+0.61}_{-0.61}$&$1.79^{+0.70}_{-0.71}$&$2.84^{+0.48}_{-1.06}$&5.81&0.05&43.5&0.42&0.40&$0.92\pm0.26$&325.04\\
201596600&177.6105&1.9911&QX&18.7&18.5&0.58&$2.71^{+0.00}_{-0.00}$&$2.58^{+0.65}_{-0.90}$&$2.71^{+0.00}_{-0.00}$&4.62&0.38&6.1&0.25&0.32&$0.48\pm0.00$&276.15\\
201598312&180.8907&2.0179&AR&15.5&12.6&0.08&$2.97^{+0.52}_{-0.94}$&$2.71^{+0.61}_{-0.96}$&$1.66^{+0.90}_{-0.90}$&1.46&0.02&78.9&0.14&0.12&$0.13\pm0.03$&29.87\\
201600065&167.1896&2.0447&AR&18.3&15.7&0.16&$1.66^{+0.28}_{-0.28}$&$1.66^{+0.00}_{-0.00}$&$1.66^{+0.05}_{-0.05}$&2.21&-0.01&12.0&2.08&2.17&$2.28\pm0.03$&5.55\\
201605601&174.1379&2.1299&AX&19.3&17.7&0.24&$3.11^{+1.07}_{-1.07}$&$3.11^{+0.98}_{-0.98}$&$2.97^{+0.97}_{-0.97}$&6.12&0.02&99.9&0.92&0.91&$1.12\pm0.87$&2.22\\
201606738&169.0130&2.1478&QR&17.3&16.8&0.21&$2.97^{+0.46}_{-0.92}$&$2.71^{+0.67}_{-0.89}$&$2.71^{+0.41}_{-0.86}$&5.42&0.03&48.9&0.87&0.89&$1.04\pm0.47$&2.47\\
201619431&171.3605&2.3442&AX&16.6&14.7&0.05&$2.18^{+0.52}_{-0.52}$&$2.18^{+0.52}_{-0.52}$&$2.32^{+0.43}_{-0.23}$&4.71&0.01&24.0&0.69&0.66&$0.68\pm0.14$&8.99\\
201619502&167.6317&2.3453&AX&18.3&17.3&0.08&$2.71^{+0.20}_{-0.53}$&$1.79^{+0.72}_{-0.48}$&$2.58^{+0.19}_{-0.56}$&5.51&0.11&14.7&1.12&1.11&$1.18\pm0.33$&0.91\\
201625264&180.6378&2.4333&QX&17.1&16.7&0.27&$2.97^{+1.19}_{-1.19}$&$2.58^{+0.72}_{-0.90}$&$2.32^{+0.62}_{-0.83}$&4.99&0.07&66.4&0.62&0.61&$0.72\pm0.27$&0.60\\
201629077&180.8873&2.4930&AR&16.0&14.2&0.08&$2.97^{+0.69}_{-0.69}$&$2.97^{+0.45}_{-0.74}$&$2.84^{+0.49}_{-0.58}$&6.07&0.01&41.6&1.18&1.08&$1.16\pm0.53$&18.58\\
201635655&170.9261&2.5956&QR&19.1&18.5&1.52&$1.92^{+0.85}_{-0.65}$&$1.53^{+0.43}_{-0.42}$&$1.92^{+0.88}_{-0.88}$&2.84&0.32&66.4&0.94&0.97&$1.48\pm0.24$&3.26\\
201637365&167.9987&2.6221&QX&18.2&18.1&1.88&$2.84^{+0.46}_{-0.90}$&$2.32^{+0.47}_{-0.44}$&$1.92^{+0.22}_{-0.48}$&2.37&0.20&18.4&0.66&0.64&$1.04\pm0.06$&215.04\\
201638033&168.7819&2.6327&QR&17.1&17.3&0.57&$2.58^{+0.00}_{-0.00}$&$2.05^{+0.82}_{-0.81}$&$2.58^{+0.00}_{-0.00}$&4.23&0.03&7.3&0.37&0.37&$0.52\pm0.00$&797.49\\
201639672&177.3290&2.6573&QR&18.8&18.1&1.54&$2.84^{+0.30}_{-0.48}$&$2.32^{+0.10}_{-0.15}$&$2.71^{+0.00}_{-0.00}$&4.91&0.98&9.4&1.45&1.36&$3.01\pm0.00$&104.50\\
201641120&171.6493&2.6795&QR&18.2&17.9&0.77&$2.45^{+0.68}_{-0.74}$&$1.92^{+0.94}_{-0.47}$&$2.71^{+0.40}_{-0.64}$&5.19&0.06&45.8&0.57&0.55&$0.90\pm0.23$&288.93\\
201649848$^{*}$&175.9610&2.8141&AX&18.7&17.9&0.28&$2.05^{+1.03}_{-0.47}$&$1.00^{+0.40}_{-0.39}$&$1.79^{+0.71}_{-0.71}$&2.38&0.23&85.7&1.31&1.35&$1.49\pm0.32$&87.69\\
201650555&168.8345&2.8246&QR&19.5&18.1&0.72&$1.53^{+0.81}_{-0.81}$&$1.00^{+0.47}_{-0.47}$&$1.39^{+0.78}_{-0.78}$&0.83&0.50&78.2&0.98&1.04&$1.16\pm0.10$&5.61\\
201654829$^{*}$&176.0345&2.8922&QR&19.2&18.5&1.28&$1.26^{+0.49}_{-0.49}$&$1.00^{+0.26}_{-0.26}$&$1.66^{+0.78}_{-0.51}$&1.89&0.41&31.6&0.89&0.90&$1.18\pm0.11$&25.51\\
201668548&175.0363&3.1198&AX&17.0&15.8&0.08&$2.05^{+0.26}_{-0.25}$&$1.92^{+0.73}_{-0.71}$&$2.05^{+0.21}_{-0.23}$&3.77&0.01&21.0&0.66&0.64&$0.67\pm0.07$&122.96\\
201676418&174.5156&3.2494&QX&18.5&18.5&2.44&$1.92^{+0.84}_{-0.62}$&$2.58^{+0.73}_{-0.81}$&$1.66^{+0.59}_{-0.23}$&1.59&0.34&24.5&0.75&0.71&$1.06\pm0.04$&0.00\\
201688660&173.3598&3.4484&QR&18.2&17.7&0.24&$2.84^{+0.42}_{-0.86}$&$2.05^{+0.60}_{-0.38}$&$2.71^{+0.61}_{-0.76}$&5.30&0.26&92.3&1.83&1.80&$2.16\pm1.02$&1.67\\
201696126&177.2083&3.5742&QR&18.9&18.3&1.48&$2.45^{+0.62}_{-0.84}$&$1.53^{+1.11}_{-1.10}$&$2.32^{+0.78}_{-0.68}$&3.89&0.19&75.8&0.62&0.65&$1.18\pm0.23$&5.68\\
201696941&173.2956&3.5880&AR&21.2&19.4&0.35&$3.11^{+0.00}_{-0.00}$&$2.18^{+0.75}_{-0.65}$&$2.97^{+0.00}_{-0.00}$&5.48&0.00&6.7&0.15&0.14&$0.19\pm0.00$&234.71\\
201697497&181.0729&3.5974&AR&18.5&15.7&0.20&$1.79^{+1.01}_{-1.01}$&$1.13^{+1.83}_{-1.83}$&$1.92^{+0.93}_{-0.93}$&1.54&0.11&97.8&0.16&0.22&$0.24\pm0.09$&1.31\\
201699775&181.2865&3.6361&AR&20.6&19.1&0.24&$2.05^{+0.94}_{-0.94}$&$2.18^{+0.88}_{-0.78}$&$2.05^{+0.89}_{-0.92}$&3.15&0.39&98.9&0.63&0.64&$0.72\pm0.28$&3.18\\
201700279&174.0557&3.6447&QR&18.6&17.8&1.19&$2.45^{+0.52}_{-0.63}$&$2.05^{+0.00}_{-0.00}$&$2.32^{+0.50}_{-0.69}$&4.19&0.07&85.9&0.55&0.57&$0.95\pm0.17$&0.94\\
201701542&171.2899&3.6653&AR&20.1&17.4&0.26&$2.18^{+0.66}_{-0.91}$&$1.13^{+0.93}_{-0.93}$&$1.79^{+0.78}_{-0.71}$&2.19&0.10&88.1&0.33&0.36&$0.39\pm0.09$&170.35\\
201703820&174.7117&3.7045&AX&18.3&16.7&0.17&$1.92^{+0.65}_{-0.63}$&$1.39^{+0.71}_{-0.70}$&$1.79^{+0.77}_{-0.61}$&2.08&0.02&83.7&0.22&0.21&$0.22\pm0.05$&1.61\\
201710297&180.4089&3.8131&AR&15.6&14.2&0.07&$2.45^{+0.52}_{-0.88}$&$2.84^{+0.32}_{-0.60}$&$2.18^{+0.55}_{-0.65}$&3.38&0.02&51.4&0.21&0.19&$0.20\pm0.07$&2.55\\
201711545&178.2856&3.8346&q&20.5&17.9&1.00&$2.45^{+0.55}_{-1.04}$&$2.32^{+0.68}_{-1.17}$&$1.92^{+0.68}_{-0.63}$&2.23&5.26&51.2&2.41&2.05&$2.82\pm0.43$&4.02\\
201711864&177.8400&3.8404&QR&18.9&18.4&2.39&$2.32^{+0.27}_{-0.74}$&$1.00^{+0.77}_{-0.77}$&$1.00^{+0.42}_{-0.42}$&-0.20&0.50&40.4&1.20&1.32&$1.32\pm0.00$&0.00\\
201714475&174.9026&3.8865&QR&18.1&17.4&0.32&$2.84^{+0.73}_{-0.73}$&$2.32^{+0.98}_{-0.91}$&$2.18^{+0.79}_{-0.51}$&3.23&0.06&81.0&0.89&0.84&$0.99\pm0.29$&23.57\\
201714961&178.4292&3.8948&q&18.0&17.7&0.70&$2.84^{+0.40}_{-0.92}$&$3.24^{+0.00}_{-0.00}$&$2.58^{+0.40}_{-0.63}$&3.89&0.16&29.9&0.70&0.68&$1.03\pm0.25$&11.54\\
201714969&172.2260&3.8948&QR&18.6&18.4&1.83&$2.58^{+0.75}_{-0.75}$&$1.92^{+0.62}_{-0.54}$&$2.32^{+0.91}_{-0.72}$&3.98&0.11&81.7&0.98&0.98&$1.95\pm0.37$&82.31\\
201719046&180.6586&3.9640&QX&18.1&17.4&0.32&$2.58^{+0.56}_{-0.83}$&$2.71^{+0.55}_{-0.94}$&$2.05^{+0.77}_{-0.67}$&3.23&0.25&88.9&0.87&0.88&$1.02\pm0.29$&524.01\\
201719625&171.7820&3.9736&QX&18.2&17.9&0.55&$2.32^{+0.52}_{-0.56}$&$2.71^{+0.46}_{-0.71}$&$2.32^{+0.63}_{-0.55}$&3.87&0.04&47.3&0.50&0.50&$0.67\pm0.17$&12.12\\
201720603&172.2336&3.9896&AX&18.5&17.9&0.18&$2.32^{+0.67}_{-0.65}$&$2.05^{+0.70}_{-0.65}$&$2.71^{+0.37}_{-0.65}$&5.05&0.12&38.3&1.86&1.72&$1.98\pm0.73$&38.31\\
201725207&176.4959&4.0694&AX&18.4&17.8&0.27&$3.11^{+1.22}_{-1.22}$&$2.05^{+1.00}_{-0.85}$&$2.97^{+1.02}_{-1.02}$&6.15&0.18&88.9&1.59&1.60&$2.03\pm1.61$&2.50\\
201725601&169.1485&4.0761&q&19.1&18.5&1.50&$1.92^{+0.53}_{-0.46}$&$1.13^{+1.90}_{-1.89}$&$1.66^{+0.43}_{-0.18}$&1.18&0.60&14.8&0.83&0.72&$0.98\pm0.04$&6.66\\
201731369&178.2071&4.1732&AR&19.2&16.3&0.13&$2.84^{+1.25}_{-1.25}$&$1.79^{+0.97}_{-0.63}$&$2.84^{+0.52}_{-1.24}$&5.31&0.05&56.9&0.21&0.20&$0.23\pm0.16$&207.58\\
201733081&170.8063&4.2025&X&18.9&17.9&0.00&$1.79^{+0.53}_{-0.47}$&$1.79^{+1.05}_{-1.05}$&$1.26^{+0.93}_{-0.91}$&0.03&0.09&45.1&0.27&0.28&$0.00\pm0.00$&0.00\\
201733246&177.1299&4.2054&q&18.5&18.4&1.50&$2.58^{+0.66}_{-1.27}$&$2.05^{+0.92}_{-0.85}$&$2.45^{+0.58}_{-1.27}$&4.46&0.63&75.0&0.72&0.68&$1.33\pm0.36$&0.82\\
201749486&171.0141&4.4747&AX&17.4&16.6&0.15&$2.45^{+0.51}_{-0.57}$&$2.45^{+0.66}_{-0.67}$&$2.32^{+0.42}_{-0.34}$&4.43&0.02&31.0&1.20&1.08&$1.18\pm0.26$&346.00\\
201751743&176.8929&4.5131&QR&19.0&18.5&1.21&$2.05^{+0.58}_{-0.76}$&$1.53^{+0.91}_{-0.91}$&$1.39^{+0.97}_{-0.97}$&0.43&0.33&42.5&0.68&0.74&$0.86\pm0.07$&4.11\\
201752000&175.1329&4.5175&q&19.5&18.5&1.00&$2.58^{+0.75}_{-1.11}$&$1.53^{+0.65}_{-0.65}$&$2.05^{+1.04}_{-0.92}$&2.11&1.15&66.5&0.72&0.77&$1.11\pm0.29$&127.54\\
201753769&173.3371&4.5487&QR&17.6&17.1&0.25&$2.05^{+0.37}_{-0.47}$&$2.05^{+0.76}_{-0.82}$&$2.05^{+0.48}_{-0.39}$&3.13&0.09&53.1&0.89&0.86&$0.97\pm0.18$&53.37\\
201756265&171.4026&4.5906&AX&18.4&17.5&0.28&$2.97^{+0.74}_{-0.74}$&$2.84^{+0.59}_{-0.54}$&$2.84^{+0.56}_{-0.99}$&5.64&0.09&91.1&0.82&0.82&$1.03\pm0.57$&10.06\\
201757807&177.3253&4.6188&q&18.8&18.3&1.40&$1.79^{+0.24}_{-0.40}$&$1.79^{+0.00}_{-0.00}$&$1.53^{+0.55}_{-0.32}$&0.40&0.59&16.5&0.58&0.62&$0.78\pm0.04$&7.05\\
201759850&177.0229&4.6540&QR&17.5&16.9&1.77&$2.84^{+0.46}_{-0.86}$&$2.32^{+0.35}_{-0.44}$&$2.18^{+0.66}_{-0.85}$&2.80&0.01&38.7&0.13&0.13&$0.24\pm0.04$&221.06\\
201762367&168.5519&4.6977&QX&18.8&18.3&0.25&$2.32^{+0.78}_{-0.86}$&$1.39^{+1.24}_{-1.23}$&$1.92^{+0.93}_{-0.62}$&2.77&0.35&85.6&1.13&1.12&$1.24\pm0.35$&1247.52\\
201768401&177.4791&4.8036&QR&17.4&16.9&0.27&$2.97^{+0.64}_{-0.65}$&$2.18^{+0.60}_{-0.49}$&$2.18^{+0.55}_{-0.55}$&3.48&0.03&82.9&0.43&0.41&$0.47\pm0.12$&4.06\\
201774618&177.1513&4.9108&q&18.5&18.2&0.60&$2.32^{+0.65}_{-0.98}$&$2.45^{+0.00}_{-0.00}$&$2.05^{+0.77}_{-0.83}$&2.71&0.40&95.7&0.89&0.83&$1.07\pm0.28$&14.25\\
201775638&177.0173&4.9269&q&19.7&18.4&1.10&$2.05^{+0.62}_{-0.72}$&$1.92^{+0.71}_{-0.65}$&$1.53^{+0.71}_{-0.71}$&0.47&1.56&63.5&0.82&1.13&$1.37\pm0.12$&37.89\\
201789585&168.8263&5.1772&AR&19.5&17.9&0.18&$2.84^{+0.50}_{-0.86}$&$1.79^{+0.46}_{-0.58}$&$2.32^{+0.64}_{-0.63}$&3.75&0.22&89.9&0.83&0.83&$0.92\pm0.33$&56.41\\
201792146&170.6709&5.2256&qX&18.0&16.9&0.20&$2.84^{+0.39}_{-0.56}$&$2.84^{+0.50}_{-0.89}$&$2.84^{+0.64}_{-0.65}$&5.31&0.05&51.5&2.64&2.45&$2.90\pm1.43$&1.22\\
201796377&170.8230&5.3012&QX&17.3&17.0&1.00&$2.97^{+0.80}_{-0.80}$&$2.32^{+0.65}_{-0.85}$&$2.58^{+0.55}_{-0.82}$&4.90&0.03&89.3&0.33&0.33&$0.57\pm0.15$&4.64\\
201805756&170.8671&5.4731&AX&18.0&17.4&0.10&$2.45^{+0.57}_{-0.53}$&$2.32^{+0.65}_{-0.79}$&$2.45^{+0.57}_{-0.52}$&5.04&0.07&82.6&1.55&1.53&$1.64\pm0.59$&339.11\\
201839008&168.6682&6.0905&q&19.2&18.4&1.20&$2.58^{+0.50}_{-0.51}$&$1.53^{+1.08}_{-1.08}$&$2.18^{+0.61}_{-0.24}$&3.44&1.11&22.2&1.38&1.36&$2.17\pm0.25$&1.19\\
201839261&168.8082&6.0951&q&18.4&18.0&0.90&$2.45^{+0.43}_{-0.51}$&$2.45^{+0.77}_{-1.08}$&$2.45^{+0.34}_{-0.64}$&4.45&0.38&27.5&0.86&0.81&$1.29\pm0.24$&105.66\\
201852752&173.5861&6.3592&QR&19.1&18.2&0.94&$1.92^{+0.63}_{-0.62}$&$1.66^{+0.73}_{-0.49}$&$2.45^{+0.51}_{-0.66}$&3.55&0.33&29.5&0.66&0.69&$1.11\pm0.24$&105.16\\
201854154&172.2160&6.3876&QR&18.2&17.0&1.49&$1.66^{+0.75}_{-0.40}$&$1.66^{+1.07}_{-1.07}$&$1.66^{+0.67}_{-0.49}$&1.28&0.08&69.9&0.49&0.48&$0.65\pm0.05$&64.41\\
201858344&172.5835&6.4744&QR&18.7&18.1&0.57&$2.45^{+0.21}_{-0.13}$&$2.58^{+0.77}_{-0.90}$&$2.32^{+0.40}_{-0.43}$&4.44&0.25&32.3&1.10&1.08&$1.46\pm0.25$&439.90\\
201859997&177.6364&6.5082&qR&18.5&18.5&2.20&$2.32^{+0.57}_{-0.64}$&$2.18^{+0.75}_{-0.75}$&$2.32^{+0.50}_{-0.57}$&4.17&0.34&42.3&0.84&0.82&$1.76\pm0.19$&29.00\\
201860527&171.5639&6.5192&q&18.9&18.5&0.90&$2.71^{+0.50}_{-0.71}$&$3.24^{+0.48}_{-0.48}$&$2.58^{+0.41}_{-0.76}$&5.27&0.00&38.0&0.12&0.12&$0.20\pm0.05$&888.78\\
201860585&174.1498&6.5204&QX&17.6&17.5&0.53&$2.97^{+0.51}_{-0.49}$&$2.71^{+0.52}_{-0.85}$&$2.45^{+0.48}_{-0.39}$&4.76&0.02&29.6&0.40&0.37&$0.50\pm0.10$&69.33\\
201863827&175.4769&6.5860&AX&17.6&16.3&0.10&$2.32^{+0.51}_{-0.51}$&$2.05^{+0.60}_{-0.62}$&$2.18^{+0.56}_{-0.47}$&3.45&0.02&73.2&0.66&0.63&$0.67\pm0.19$&58.12\\
201886269&178.1653&7.0394&QX&17.9&17.4&1.49&$2.97^{+0.66}_{-0.66}$&$2.18^{+0.38}_{-0.50}$&$2.45^{+0.38}_{-0.94}$&4.12&0.10&21.3&0.38&0.36&$0.70\pm0.13$&1.64\\
201889930&175.2542&7.1137&q&18.9&18.2&1.00&$2.45^{+0.62}_{-0.63}$&$2.05^{+0.64}_{-0.82}$&$2.58^{+0.58}_{-0.69}$&4.74&0.80&51.1&0.91&0.96&$1.66\pm0.42$&562.95\\
201889976&175.3575&7.1146&Q&18.1&17.7&0.50&$3.11^{+0.37}_{-0.45}$&$1.92^{+0.74}_{-0.36}$&$3.24^{+0.10}_{-0.27}$&5.79&0.20&11.6&0.69&0.69&$1.08\pm0.15$&87.78\\
201894176&176.0200&7.2015&QX&18.1&17.6&0.50&$2.97^{+0.52}_{-0.82}$&$2.97^{+0.00}_{-0.00}$&$2.97^{+0.44}_{-0.78}$&5.48&0.16&40.9&1.02&1.00&$1.49\pm0.60$&33.64\\
201905730&177.0650&7.4441&QR&18.7&18.2&2.21&$2.32^{+0.76}_{-0.91}$&$2.45^{+0.70}_{-0.56}$&$1.66^{+0.60}_{-0.51}$&1.32&0.52&37.9&0.55&0.69&$1.01\pm0.06$&0.00\\
201909148&175.1983&7.5162&AX&17.3&16.2&0.13&$2.58^{+0.48}_{-0.69}$&$2.71^{+0.52}_{-1.02}$&$2.45^{+0.54}_{-0.60}$&4.02&0.04&76.1&1.04&1.00&$1.09\pm0.40$&33.48\\
201910112&172.5724&7.5369&QR&17.6&17.4&2.66&$2.32^{+0.63}_{-0.91}$&$1.79^{+0.65}_{-0.37}$&$2.58^{+0.27}_{-0.63}$&4.72&0.06&25.0&0.32&0.30&$0.82\pm0.08$&0.00\\
202059522&102.6933&25.0499&BR&17.1&16.6&0.20&$2.18^{+0.34}_{-0.18}$&$2.32^{+0.19}_{-0.14}$&$2.18^{+0.33}_{-0.24}$&4.03&-0.02&21.7&1.76&1.60&$1.78\pm0.25$&3.29\\
202064584&101.3162&21.4139&X&17.8&17.1&0.00&$1.92^{+0.85}_{-0.77}$&$3.37^{+0.00}_{-0.00}$&$1.79^{+0.89}_{-0.66}$&2.38&0.04&57.1&0.48&0.47&$0.00\pm0.00$&0.00\\
202064619&98.9237&27.9006&q&19.4&17.8&1.00&$3.24^{+0.00}_{-0.00}$&$1.00^{+0.00}_{-0.00}$&$2.97^{+0.00}_{-0.00}$&4.36&6.02&3.2&-&0.58&$1.15\pm0.00$&9.70\\
202064620&94.1183&24.7217&q&18.0&17.8&1.20&$1.79^{+1.63}_{-1.62}$&$2.18^{+1.26}_{-1.26}$&$2.18^{+1.32}_{-0.99}$&2.22&13.78&72.3&1.71&2.28&$3.64\pm1.13$&57.96\\
202064700&94.2358&24.6472&q&18.3&18.2&1.40&$2.84^{+1.27}_{-1.27}$&$1.00^{+2.44}_{-2.31}$&$2.97^{+1.39}_{-1.39}$&4.68&2.30&58.7&1.52&1.72&$4.07\pm2.32$&291.27\\
202064759&98.1854&27.9022&q&19.8&18.4&0.80&$1.13^{+1.04}_{-1.04}$&$2.58^{+0.54}_{-0.49}$&$1.00^{+1.26}_{-1.26}$&-0.96&0.03&23.4&0.15&0.09&$0.09\pm0.00$&338.44\\
202064761&101.3950&28.8364&q&18.7&18.4&2.40&$2.97^{+0.00}_{-0.00}$&$2.05^{+0.79}_{-0.96}$&$2.71^{+0.04}_{-0.08}$&4.80&0.27&10.8&0.49&0.55&$1.56\pm0.02$&0.00\\
202064763&92.8396&22.9825&q&18.7&18.4&1.10&$1.66^{+1.40}_{-1.40}$&$1.79^{+1.39}_{-1.38}$&$1.26^{+1.79}_{-1.79}$&0.23&0.01&86.0&0.13&0.14&$0.16\pm0.02$&25.55\\
202064787&97.0787&25.4114&q&18.5&18.4&2.10&$2.05^{+0.68}_{-0.97}$&$2.58^{+0.50}_{-0.50}$&$1.79^{+0.88}_{-0.73}$&2.05&0.42&42.0&0.74&0.74&$1.16\pm0.12$&129.78\\
202064867&99.7871&27.4075&q&19.0&18.7&1.20&$2.97^{+0.48}_{-0.60}$&$2.32^{+0.78}_{-0.86}$&$2.71^{+0.76}_{-1.14}$&4.78&0.02&69.7&0.31&0.30&$0.60\pm0.22$&791.48\\
202064872&96.3129&26.4617&q&20.0&18.7&0.70&$2.97^{+0.23}_{-1.72}$&$1.39^{+0.39}_{-0.21}$&$1.39^{+1.78}_{-1.78}$&0.47&2.46&31.3&1.73&1.85&$2.05\pm0.42$&124.95\\
202064880&93.1933&24.6111&q&18.8&18.7&1.40&$3.11^{+1.27}_{-1.28}$&$1.26^{+2.07}_{-2.05}$&$2.84^{+0.47}_{-1.19}$&5.65&6.33&28.0&2.98&2.97&$6.66\pm2.12$&16.04\\
202064932&103.7400&24.1011&QR&18.7&18.8&0.00&$3.24^{+0.58}_{-0.58}$&$2.71^{+1.64}_{-1.64}$&$2.84^{+1.67}_{-1.67}$&5.53&0.76&69.5&0.93&1.00&$0.00\pm0.00$&0.00\\
202064938&98.0033&26.7303&q&20.2&18.8&0.40&$1.66^{+1.26}_{-1.26}$&$1.13^{+1.31}_{-1.31}$&$1.66^{+1.33}_{-1.33}$&1.39&5.14&97.5&2.74&2.77&$3.09\pm0.97$&221.06\\
202064941&99.0879&28.0328&qR&19.5&18.8&2.30&$2.71^{+0.45}_{-1.24}$&$3.24^{+0.00}_{-0.00}$&$2.71^{+0.50}_{-1.33}$&4.60&1.51&21.3&0.98&0.49&$1.35\pm0.32$&0.00\\
202064942&100.0558&28.3078&q&19.6&18.8&0.90&$1.13^{+0.88}_{-0.88}$&$1.13^{+0.49}_{-0.49}$&$1.13^{+0.86}_{-0.86}$&0.28&0.03&98.3&0.62&0.65&$0.67\pm0.02$&3.80\\
202064943&94.2192&22.7114&X&19.5&18.8&0.00&$2.45^{+0.64}_{-0.66}$&$2.84^{+0.52}_{-0.66}$&$2.58^{+0.41}_{-0.63}$&5.30&0.45&21.4&1.18&1.26&$0.00\pm0.00$&0.00\\
202064947&94.5567&24.8708&q&18.8&18.8&1.80&$2.32^{+0.56}_{-0.52}$&$2.58^{+0.35}_{-0.67}$&$2.32^{+0.49}_{-0.57}$&3.93&0.00&61.2&0.23&0.21&$0.42\pm0.05$&38.93\\
202065012&97.5071&25.2339&q&20.4&18.9&0.80&$3.11^{+0.21}_{-0.21}$&$1.66^{+1.33}_{-1.32}$&$3.11^{+0.47}_{-0.47}$&5.86&2.55&38.4&4.88&4.88&$9.07\pm2.50$&424.82\\
202065014&96.5279&24.5553&q&20.3&18.9&1.80&$2.84^{+0.37}_{-1.24}$&$2.58^{+0.56}_{-1.08}$&$2.97^{+0.34}_{-1.19}$&6.02&0.14&27.5&0.60&0.64&$1.78\pm0.48$&15.75\\
202065018&99.1083&27.3522&q&19.6&18.9&0.00&$2.58^{+0.57}_{-1.15}$&$2.84^{+0.56}_{-0.82}$&$2.05^{+0.91}_{-0.91}$&2.79&0.03&99.2&0.29&0.29&$0.00\pm0.00$&0.00\\
202065020&95.4704&24.8564&qR&20.2&18.9&0.50&$2.84^{+0.43}_{-0.42}$&$1.66^{+1.32}_{-1.32}$&$2.84^{+0.38}_{-0.38}$&5.05&2.16&25.2&1.28&0.93&$1.35\pm0.31$&118.93\\
202065024&97.2104&27.5569&q&20.0&18.9&1.10&$2.97^{+0.52}_{-0.51}$&$1.13^{+1.02}_{-1.01}$&$2.84^{+0.61}_{-0.61}$&4.45&2.69&32.5&0.89&0.62&$1.22\pm0.33$&6.29\\
202065027&95.2908&26.3306&q&20.3&18.9&2.20&$3.11^{+1.77}_{-1.77}$&$1.92^{+1.52}_{-1.51}$&$1.79^{+0.76}_{-0.76}$&1.70&0.03&50.2&0.20&0.21&$0.33\pm0.03$&44.06\\
202065033&92.6587&24.0169&q&19.0&18.9&0.90&$1.79^{+1.41}_{-1.41}$&$2.05^{+1.04}_{-1.04}$&$1.26^{+1.79}_{-1.79}$&-0.11&0.09&82.6&0.26&0.25&$0.28\pm0.03$&189.93\\
203712498&238.8386&-25.1987&X&17.9&17.6&0.00&$2.71^{+0.00}_{-0.00}$&$2.18^{+0.00}_{-0.00}$&$2.05^{+0.72}_{-0.88}$&2.98&2.95&65.9&1.77&1.74&$0.00\pm0.00$&0.00\\
204364577&243.6638&-22.6238&X&19.6&18.8&0.00&$2.45^{+0.32}_{-0.65}$&$2.05^{+0.00}_{-0.00}$&$1.66^{+0.83}_{-0.50}$&1.59&0.28&21.4&0.81&0.77&$0.00\pm0.00$&0.00\\
205069410&240.2535&-19.5551&q&20.5&18.8&1.20&$2.18^{+0.00}_{-0.00}$&$2.05^{+0.47}_{-0.30}$&$2.58^{+0.55}_{-1.14}$&4.44&3.45&42.4&1.38&1.37&$2.55\pm0.77$&63.81\\
205108579&242.0021&-19.3619&q&19.0&17.8&2.40&$2.18^{+0.00}_{-0.00}$&$1.66^{+0.63}_{-0.63}$&$1.53^{+0.77}_{-0.45}$&1.33&0.01&46.4&0.12&0.12&$0.17\pm0.01$&0.00\\
205161826&240.3796&-19.0947&q&19.7&18.6&1.20&$2.32^{+0.00}_{-0.00}$&$1.53^{+0.90}_{-0.90}$&$2.05^{+0.64}_{-0.92}$&2.50&0.18&86.8&0.26&0.37&$0.56\pm0.11$&36.04\\
205233430&239.9710&-18.7242&q&19.5&18.8&1.00&$2.32^{+0.00}_{-0.00}$&$1.26^{+0.69}_{-0.69}$&$1.00^{+0.00}_{-0.00}$&-0.41&5.10&2.8&3.10&2.96&$2.96\pm0.00$&69.66\\
205499024&242.1542&-17.1865&q&19.5&19.0&1.00&$1.39^{+0.00}_{-0.00}$&$1.79^{+0.24}_{-0.18}$&$1.39^{+0.00}_{-0.00}$&0.72&8.21&0.9&5.49&4.99&$5.72\pm0.00$&53.37\\
205589571&243.0043&-16.5535&q&19.2&18.5&2.30&$2.32^{+0.00}_{-0.00}$&$2.32^{+0.00}_{-0.00}$&$1.53^{+0.63}_{-0.63}$&1.10&0.50&84.9&0.97&0.95&$1.30\pm0.07$&0.00\\
205657421&241.6560&-16.0313&q&19.6&18.8&0.90&$2.05^{+0.17}_{-0.14}$&$1.79^{+0.83}_{-0.62}$&$1.66^{+0.52}_{-0.52}$&1.26&4.22&56.6&1.22&1.63&$2.02\pm0.18$&53.37\\
205662407&242.2596&-15.9916&q&20.0&18.7&1.40&$2.32^{+0.63}_{-0.63}$&$1.92^{+0.50}_{-0.67}$&$2.32^{+0.28}_{-0.25}$&4.02&1.05&17.2&4.06&3.75&$6.67\pm0.48$&38.93\\
205708067&248.0279&-15.6024&2&19.5&19.0&0.00&$2.05^{+0.00}_{-0.00}$&$2.58^{+0.62}_{-0.90}$&$2.45^{+0.60}_{-0.99}$&4.21&0.03&77.0&0.31&0.29&$0.00\pm0.00$&0.00\\
205905563&333.4540&-17.9759&QX&17.6&17.6&1.18&$3.11^{+0.00}_{-0.00}$&$2.71^{+0.00}_{-0.00}$&$2.84^{+0.00}_{-0.00}$&5.62&1.05&1.4&1.90&1.69&$3.47\pm0.00$&80.61\\
205922171&339.6602&-17.3434&X&17.1&18.2&0.00&$2.71^{+0.57}_{-0.97}$&$2.58^{+0.54}_{-0.83}$&$2.58^{+0.69}_{-0.82}$&5.26&0.21&66.7&1.37&1.34&$0.00\pm0.00$&0.00\\
205926751&333.2510&-17.1716&AR&17.2&16.6&0.15&$2.84^{+0.42}_{-0.85}$&$2.05^{+0.49}_{-0.36}$&$2.32^{+0.47}_{-0.51}$&3.77&0.03&67.3&1.01&1.03&$1.12\pm0.31$&393.09\\
205951387&333.7327&-16.3245&AX&18.2&17.0&0.30&$2.58^{+0.68}_{-0.85}$&$2.18^{+0.38}_{-0.61}$&$2.45^{+0.73}_{-0.80}$&3.98&0.05&94.8&1.13&1.12&$1.35\pm0.58$&4.49\\
205955477&333.8638&-16.1925&QX&20.6&18.1&3.99&$2.97^{+0.14}_{-0.96}$&$1.00^{+1.10}_{-1.10}$&$2.05^{+0.47}_{-0.32}$&3.23&0.19&28.7&1.39&1.39&$3.24\pm0.14$&0.00\\
206015673&337.9152&-14.3728&R&17.5&17.3&0.00&$2.97^{+0.81}_{-0.81}$&$1.79^{+0.68}_{-0.51}$&$2.18^{+0.63}_{-0.69}$&3.33&0.07&70.5&0.41&0.42&$0.00\pm0.00$&0.00\\
206020795&343.2466&-14.2231&X&18.6&18.2&0.00&$2.97^{+0.24}_{-0.23}$&$2.84^{+0.17}_{-0.07}$&$2.84^{+0.37}_{-0.20}$&5.89&0.40&17.6&4.62&4.01&$0.00\pm0.00$&0.00\\
206026285&331.3400&-14.0664&R&18.4&18.0&0.00&$2.97^{+0.22}_{-0.95}$&$2.97^{+0.53}_{-0.74}$&$2.32^{+0.72}_{-0.56}$&4.00&0.13&58.2&1.15&1.14&$0.00\pm0.00$&0.00\\
206065686&342.2947&-13.0008&BR&18.7&18.6&0.00&$2.97^{+0.45}_{-0.83}$&$2.71^{+0.46}_{-0.73}$&$2.45^{+0.36}_{-0.48}$&4.27&0.84&46.8&3.06&3.13&$0.00\pm0.00$&0.00\\
206172695&342.0730&-10.2631&QR&17.9&17.0&0.29&$3.11^{+0.81}_{-0.81}$&$1.39^{+0.43}_{-0.32}$&$1.92^{+0.64}_{-0.52}$&2.80&0.06&76.6&1.23&1.22&$1.37\pm0.28$&9.28\\
206185225&344.3293&-10.0180&QX&18.3&18.2&2.08&$2.45^{+0.73}_{-0.70}$&$1.92^{+0.85}_{-0.90}$&$1.66^{+0.58}_{-0.58}$&1.48&0.23&89.9&0.75&0.76&$1.10\pm0.07$&11.41\\
206191531&339.0297&-9.9036&q&18.7&18.6&1.10&$2.05^{+0.59}_{-0.59}$&$1.92^{+0.62}_{-0.54}$&$1.92^{+0.53}_{-0.43}$&1.96&0.27&72.3&1.14&1.19&$1.68\pm0.18$&920.75\\
206201587$^{*}$&337.9927&-9.7333&QR&17.8&17.8&0.92&$2.18^{+0.91}_{-0.42}$&$1.39^{+0.43}_{-0.43}$&$1.92^{+0.52}_{-0.52}$&2.74&0.01&85.3&0.72&0.73&$0.98\pm0.12$&129.78\\
206223915&340.1788&-9.3809&q&18.5&18.5&1.20&$2.05^{+0.59}_{-0.42}$&$2.18^{+0.37}_{-0.36}$&$2.05^{+0.35}_{-0.45}$&2.66&0.17&35.0&0.98&0.99&$1.50\pm0.14$&182.20\\
206224059&332.9969&-9.3786&q&18.5&18.7&2.00&$2.18^{+0.38}_{-0.31}$&$2.18^{+0.00}_{-0.00}$&$2.05^{+0.11}_{-0.13}$&3.39&0.19&12.1&0.85&0.87&$1.56\pm0.03$&190.46\\
206225059$^{*}$&338.6586&-9.3629&AR&18.9&17.8&0.25&$3.11^{+1.00}_{-1.00}$&$2.45^{+0.61}_{-0.72}$&$3.11^{+1.01}_{-1.01}$&6.07&0.12&90.2&1.45&1.46&$1.84\pm1.57$&707.23\\
206238354&339.6081&-9.1659&q&18.4&18.1&0.60&$2.84^{+0.85}_{-0.85}$&$3.37^{+0.00}_{-0.00}$&$2.45^{+0.68}_{-0.63}$&4.25&0.07&92.5&0.71&0.72&$1.02\pm0.30$&3.60\\
206240592&343.7932&-9.1320&Q2&19.9&18.4&0.41&$2.58^{+0.55}_{-0.73}$&$2.45^{+0.53}_{-0.92}$&$2.18^{+0.62}_{-0.56}$&3.64&1.41&64.0&2.07&2.23&$2.74\pm0.68$&41.13\\
206241448&334.3584&-9.1183&BR&14.1&12.6&0.09&$2.05^{+0.37}_{-0.34}$&$1.79^{+0.46}_{-0.50}$&$1.53^{+0.00}_{-0.00}$&1.79&0.00&2.2&0.26&0.23&$0.23\pm0.00$&5.12\\
206252148&342.8421&-8.9564&AR&18.4&17.3&0.08&$3.24^{+0.34}_{-0.34}$&$1.66^{+1.07}_{-1.07}$&$2.18^{+0.79}_{-0.89}$&3.19&0.14&83.6&0.54&0.54&$0.57\pm0.26$&21.63\\
206256982&334.6746&-8.8848&QR&18.3&18.0&0.76&$2.18^{+0.37}_{-0.62}$&$1.66^{+0.70}_{-0.70}$&$1.66^{+0.38}_{-0.44}$&1.20&0.17&28.2&0.43&0.46&$0.56\pm0.04$&0.57\\
206265146&334.3810&-8.7605&AR&19.3&17.8&0.16&$2.18^{+0.42}_{-0.32}$&$1.79^{+0.35}_{-0.31}$&$1.66^{+0.00}_{-0.00}$&1.97&0.07&2.8&0.43&0.42&$0.44\pm0.00$&77.28\\
206267233$^{*}$&338.2612&-8.7303&AR&17.3&15.5&0.06&$2.71^{+0.60}_{-0.94}$&$1.26^{+0.57}_{-0.57}$&$2.45^{+0.60}_{-0.60}$&4.44&0.02&94.5&0.66&0.63&$0.65\pm0.27$&1.04\\
206293494&334.3440&-8.3394&QX&19.7&18.2&1.16&$3.37^{+0.75}_{-0.75}$&$3.37^{+0.84}_{-0.84}$&$2.18^{+0.64}_{-0.62}$&3.51&0.07&69.0&1.49&1.52&$2.39\pm0.41$&0.72\\
206297540&330.1917&-8.2790&q&19.2&18.0&1.80&$2.45^{+0.50}_{-0.62}$&$2.18^{+0.00}_{-0.00}$&$2.05^{+0.64}_{-0.58}$&2.71&0.44&75.0&1.10&1.07&$1.85\pm0.21$&64.14\\
206302006&334.3315&-8.2096&QX&20.1&18.5&1.46&$2.32^{+0.80}_{-0.86}$&$2.58^{+0.53}_{-1.25}$&$1.39^{+0.88}_{-0.88}$&0.41&1.05&90.9&1.35&1.32&$1.57\pm0.11$&301.69\\
206302744&334.3726&-8.1986&QX&20.0&18.7&1.01&$1.26^{+1.02}_{-1.02}$&$1.39^{+0.65}_{-0.65}$&$1.39^{+0.96}_{-0.96}$&0.73&0.47&95.8&0.94&1.03&$1.18\pm0.11$&82.98\\
206304512$^{*}$&337.5436&-8.1717&Q&18.0&17.9&0.62&$2.05^{+0.31}_{-0.29}$&$2.05^{+0.40}_{-0.32}$&$2.05^{+0.30}_{-0.17}$&3.79&0.08&15.8&3.20&3.11&$4.01\pm0.31$&36.21\\
206315574&331.1682&-7.9991&q&19.3&18.4&1.10&$3.11^{+0.00}_{-0.00}$&$1.13^{+0.59}_{-0.59}$&$1.39^{+0.00}_{-0.00}$&0.28&55.15&2.5&5.83&7.69&$8.91\pm0.00$&61.72\\
206322522&335.2323&-7.8883&AX&17.3&17.2&0.15&$2.58^{+0.59}_{-0.64}$&$2.18^{+0.71}_{-0.60}$&$2.45^{+0.60}_{-0.55}$&4.65&0.00&44.8&0.27&0.28&$0.31\pm0.11$&78.59\\
206322600&334.4833&-7.8871&QX&19.1&18.4&1.56&$1.92^{+0.68}_{-0.84}$&$1.53^{+0.80}_{-0.80}$&$1.79^{+0.85}_{-0.67}$&2.30&0.19&95.9&0.60&0.63&$0.92\pm0.11$&4.33\\
206339230&330.8481&-7.6252&AR&14.2&11.2&0.04&$2.05^{+0.53}_{-0.34}$&$2.18^{+0.00}_{-0.00}$&$1.92^{+0.19}_{-0.17}$&2.86&0.00&15.3&0.25&0.25&$0.26\pm0.02$&230.51\\
206341987&333.0146&-7.5789&AR&14.4&11.8&0.05&$1.79^{+0.33}_{-0.32}$&$3.24^{+0.00}_{-0.00}$&$1.79^{+0.27}_{-0.29}$&2.48&0.00&23.2&0.17&0.18&$0.19\pm0.02$&4.67\\
206343765$^{*}$&337.6033&-7.5510&AR&17.5&15.6&0.06&$2.18^{+0.00}_{-0.00}$&$2.45^{+0.00}_{-0.00}$&$2.18^{+0.00}_{-0.00}$&3.94&0.01&6.2&0.56&0.51&$0.53\pm0.00$&5.82\\
206344400&330.6410&-7.5403&AR&16.0&13.4&0.06&$2.58^{+0.44}_{-0.60}$&$2.71^{+0.39}_{-0.83}$&$2.45^{+0.47}_{-0.47}$&4.54&0.01&61.5&0.90&0.86&$0.90\pm0.29$&0.59\\
206357066&338.4871&-7.3318&q&19.6&18.7&1.30&$2.05^{+0.71}_{-0.68}$&$1.26^{+0.99}_{-0.99}$&$1.66^{+0.50}_{-0.57}$&1.54&0.97&61.1&1.15&1.23&$1.62\pm0.12$&1.99\\
206357549&336.2189&-7.3233&q&18.6&18.3&0.50&$2.84^{+0.60}_{-0.89}$&$2.05^{+0.00}_{-0.00}$&$1.92^{+0.63}_{-0.47}$&3.02&0.07&76.3&0.76&0.75&$0.91\pm0.15$&92.13\\
206371473&332.6909&-7.0939&q&19.1&18.4&2.20&$1.39^{+0.36}_{-0.39}$&$1.00^{+0.43}_{-0.43}$&$1.13^{+0.36}_{-0.36}$&0.20&0.11&47.5&1.45&1.44&$1.56\pm0.01$&22.52\\
206375071&334.1738&-7.0333&q&19.0&18.6&0.20&$2.45^{+0.25}_{-0.24}$&$2.97^{+0.00}_{-0.00}$&$2.32^{+0.28}_{-0.17}$&3.62&1.10&13.6&2.62&2.52&$2.84\pm0.35$&529.16\\
206377690&337.3884&-6.9922&q&18.8&18.5&1.90&$2.71^{+0.87}_{-0.87}$&$1.66^{+0.40}_{-0.48}$&$2.58^{+0.57}_{-0.90}$&4.31&0.17&76.8&0.92&0.91&$2.11\pm0.42$&2.14\\
206379076&333.2291&-6.9694&q&18.9&18.3&0.90&$1.26^{+0.61}_{-0.61}$&$2.84^{+0.00}_{-0.00}$&$1.00^{+0.36}_{-0.36}$&0.32&-0.08&51.1&2.07&2.11&$2.11\pm0.00$&485.19\\
206391511&336.0164&-6.7706&q&18.5&18.7&1.60&$2.18^{+0.88}_{-0.49}$&$2.32^{+0.18}_{-0.34}$&$2.18^{+0.84}_{-0.42}$&3.64&0.26&29.9&1.12&1.10&$1.94\pm0.28$&69.33\\
206393145&333.3676&-6.7443&q&19.1&18.1&1.30&$1.79^{+0.00}_{-0.00}$&$1.92^{+0.52}_{-0.35}$&$1.66^{+0.00}_{-0.00}$&1.30&0.44&5.2&2.32&2.21&$2.90\pm0.00$&411.90\\
206393444&332.3568&-6.7391&qR&19.3&18.4&1.90&$2.84^{+0.52}_{-0.83}$&$2.32^{+0.33}_{-0.35}$&$1.79^{+0.58}_{-0.50}$&1.86&0.50&56.7&1.52&1.55&$2.35\pm0.17$&140.08\\
206400807&334.3470&-6.6192&q&19.3&18.7&0.70&$1.00^{+0.47}_{-0.47}$&$1.00^{+0.27}_{-0.26}$&$1.00^{+0.51}_{-0.51}$&0.34&-0.22&67.3&2.79&3.03&$3.03\pm0.00$&316.10\\
206403979&332.8894&-6.5686&qR&19.4&18.2&2.70&$1.79^{+0.50}_{-0.23}$&$1.66^{+0.26}_{-0.23}$&$1.92^{+0.19}_{-0.37}$&2.18&0.44&25.5&1.34&1.41&$2.58\pm0.09$&0.00\\
206406129&334.0766&-6.5328&q&18.4&18.0&2.20&$1.00^{+0.00}_{-0.00}$&$1.26^{+1.36}_{-1.35}$&$1.00^{+0.00}_{-0.00}$&0.14&1.38&0.6&4.51&4.87&$4.87\pm0.00$&28.23\\
206409156&337.0962&-6.4818&q&18.8&18.3&0.70&$2.58^{+0.40}_{-0.64}$&$2.58^{+0.50}_{-0.96}$&$2.45^{+0.46}_{-0.57}$&4.51&0.22&29.6&1.38&1.30&$1.91\pm0.42$&969.37\\
206411085&332.8818&-6.4500&q&19.8&18.5&1.40&$1.53^{+0.34}_{-0.34}$&$1.53^{+0.73}_{-0.73}$&$1.53^{+0.27}_{-0.31}$&1.51&2.13&23.9&3.21&3.23&$4.07\pm0.13$&42.48\\
206411765&333.6097&-6.4388&q&19.0&18.5&0.60&$2.58^{+0.69}_{-0.97}$&$2.58^{+0.59}_{-0.85}$&$2.32^{+0.61}_{-0.83}$&4.14&0.05&98.2&0.57&0.57&$0.78\pm0.23$&95.24\\
206415643&333.0105&-6.3742&q&19.4&18.4&1.90&$2.84^{+0.57}_{-1.05}$&$2.84^{+0.53}_{-1.17}$&$1.92^{+0.86}_{-0.68}$&2.84&0.58&100.0&1.54&1.56&$2.55\pm0.31$&25.21\\
206417966&332.7875&-6.3346&q&19.0&17.9&2.20&$1.79^{+0.15}_{-0.25}$&$1.53^{+0.77}_{-0.77}$&$1.92^{+0.16}_{-0.21}$&2.69&0.36&14.0&1.57&1.58&$2.70\pm0.07$&290.24\\
206431611&338.9928&-6.1068&q&18.7&18.4&1.50&$1.92^{+1.12}_{-0.38}$&$1.92^{+0.29}_{-0.36}$&$2.84^{+0.40}_{-1.27}$&5.34&0.32&29.2&1.02&1.01&$2.35\pm0.72$&576.77\\
206444031&335.2122&-5.9041&q&18.5&18.5&0.50&$1.53^{+0.15}_{-0.15}$&$1.39^{+0.55}_{-0.55}$&$1.53^{+0.00}_{-0.00}$&1.63&0.21&6.5&1.76&1.60&$1.78\pm0.00$&291.67\\
206444462&339.6827&-5.8975&q&19.0&18.5&2.00&$2.97^{+0.36}_{-0.64}$&$2.18^{+0.45}_{-0.43}$&$2.71^{+0.31}_{-0.55}$&4.70&0.33&27.5&0.94&1.00&$2.55\pm0.31$&24.41\\
206445142&338.6208&-5.8855&q&18.4&17.6&0.90&$2.32^{+0.16}_{-0.16}$&$2.45^{+0.67}_{-0.76}$&$2.05^{+0.00}_{-0.00}$&3.50&0.07&3.5&1.44&1.35&$1.89\pm0.00$&459.61\\
206455495&333.0035&-5.7121&q&19.7&18.6&0.30&$2.84^{+1.05}_{-1.05}$&$1.79^{+0.66}_{-0.76}$&$2.58^{+0.61}_{-1.04}$&4.59&2.50&87.4&3.00&2.99&$3.67\pm1.84$&105.16\\
206458738&339.7395&-5.6557&QR&18.1&16.1&0.17&$2.71^{+0.56}_{-0.98}$&$1.92^{+0.34}_{-0.19}$&$2.58^{+0.78}_{-0.79}$&4.92&0.04&56.0&0.53&0.53&$0.60\pm0.32$&2.96\\
206460591&332.5498&-5.6238&q&19.8&18.6&2.50&$2.71^{+0.46}_{-0.89}$&$1.00^{+1.64}_{-1.64}$&$2.05^{+0.57}_{-0.41}$&3.08&2.31&35.0&4.05&4.02&$7.77\pm0.57$&0.00\\
206479772&338.6594&-5.2769&q&18.3&18.6&2.00&$2.05^{+0.00}_{-0.00}$&$1.79^{+0.80}_{-0.80}$&$1.92^{+0.00}_{-0.00}$&2.29&0.62&7.2&1.39&1.26&$2.10\pm0.00$&3.20\\
206481042&335.7698&-5.2529&q&19.2&18.6&1.70&$2.45^{+0.68}_{-0.84}$&$2.18^{+0.52}_{-0.57}$&$1.92^{+0.47}_{-0.62}$&2.12&0.67&61.2&1.13&1.21&$1.91\pm0.18$&840.92\\
206491828&336.5714&-5.0429&QX&19.1&18.7&1.87&$3.37^{+0.73}_{-0.73}$&$3.11^{+0.48}_{-0.48}$&$2.58^{+0.47}_{-0.67}$&5.24&0.00&75.0&0.25&0.25&$0.58\pm0.09$&262.51\\
206495717&336.2509&-4.9649&qX&19.3&18.6&0.30&$2.97^{+0.43}_{-0.40}$&$2.18^{+0.58}_{-0.59}$&$2.32^{+0.45}_{-0.51}$&3.59&1.06&39.7&1.38&1.48&$1.76\pm0.43$&358.83\\
206496452&336.4469&-4.9504&QR&18.8&17.2&1.40&$3.11^{+1.04}_{-1.04}$&$2.58^{+0.42}_{-0.08}$&$2.71^{+0.54}_{-1.12}$&4.74&0.55&84.9&1.50&1.50&$3.17\pm0.94$&4.04\\
206506250&339.8153&-4.7517&q&19.2&18.5&1.20&$2.45^{+0.48}_{-0.68}$&$2.18^{+0.55}_{-0.61}$&$2.32^{+0.62}_{-0.56}$&3.74&0.58&54.7&1.37&1.37&$2.30\pm0.41$&222.81\\
206507165&340.3049&-4.7331&q&18.7&18.4&1.20&$1.92^{+0.00}_{-0.00}$&$1.26^{+0.74}_{-0.74}$&$1.79^{+0.19}_{-0.29}$&1.96&0.69&15.8&1.19&1.26&$1.72\pm0.07$&105.66\\
206511385&340.0497&-4.6477&X&18.6&17.9&0.00&$2.18^{+0.66}_{-0.34}$&$2.18^{+0.64}_{-0.63}$&$2.18^{+0.24}_{-0.22}$&4.10&0.11&23.6&1.09&1.09&$0.00\pm0.0$&0.00\\
206512266&335.7320&-4.6302&q&19.2&18.5&0.90&$2.32^{+0.57}_{-0.82}$&$1.39^{+0.70}_{-0.69}$&$1.79^{+0.55}_{-0.54}$&2.03&0.19&48.1&0.78&0.75&$0.97\pm0.11$&160.84\\
206530319&335.6790&-4.2460&q&19.0&18.4&1.30&$2.18^{+0.72}_{-0.51}$&$1.92^{+0.71}_{-0.59}$&$2.18^{+0.85}_{-0.46}$&3.53&0.42&27.7&1.61&1.58&$2.58\pm0.44$&54.09\\

